Geometric Fabrics for the Acceleration-based Design of Robotic Motion

This paper describes the pragmatic design and construction of geometric fabrics for shaping a robot's task-independent nominal behavior, capturing behavioral components such as obstacle avoidance, joint limit avoidance, redundancy resolution, global navigation heuristics, etc. Geometric fabrics constitute the most concrete incarnation of a new mathematical formulation for reactive behavior called optimization fabrics. Fabrics generalize recent work on Riemannian Motion Policies (RMPs); they add provable stability guarantees and improve design consistency while promoting the intuitive acceleration-based principles of modular design that make RMPs successful. We describe a suite of mathematical modeling tools that practitioners can employ in practice and demonstrate both how to mitigate system complexity by constructing behaviors layer-wise and how to employ these tools to design robust, strongly-generalizing, policies that solve practical problems one would expect to find in industry applications. Our system exhibits intelligent global navigation behaviors expressed entirely as provably stable fabrics with zero planning or state machine governance.

==> geometric_fabrics/8_particle_experiments.tex <==
% \fullversiononly

% \section{Empirical validation of theoretical results}

% \nathan{Add introductory sentence saying that we're verifying / demonstrating empirically some of the theroetical results we derived above.}

% \subsection{Path Consistency of Geometries} \label{sec:PathConsistencyExperiment}
% To illustrate that geometries under the generator equation, $\xdd + \h_2(\q, \qd) = 0$, produce consistent paths given initial conditions, $(\q_0, \alpha \hat{\qd}_0)$, a set of obstacle avoiding geometries are designed and integrated forward. For each designed geometry, two different values of $\alpha$ are used to show that the yielded paths are exactly the same. The results also show the flexibility in defining geometries which can be leveraged to enable desired behavior.

% A geometry $\h_2(\q, \qd)$ that naturally produces particle paths that avoid obstacles can be defined in coordinates, $\q \in \mathbb{R}^{2}$, as 
% \begin{align} \label{eqn: phi2_case1}
%     \h_2(\q,\qd) = \lambda \| \qd \| ^2 \: \partial_\q \psi(\phi(\q))
% \end{align}
% where $\phi(\q)$ is a differentiable map that captures the distance to a circular object and $\lambda \in \mathbb{R}^+$ is a scaling gain. More specifically, $\phi(\q) = \frac{\|\q - \q_o\| - r}{r}$, where $\q_o$ and $r$ are the circle's center and radius, respectively. Furthermore, $\psi(\phi(\q)) \in \mathbb{R}^+$ is a barrier potential function, $\psi(\phi(\q)) = \frac{k}{\phi(\q)^2}$, where $k \in \mathbb{R}^+$ is a scaling gain. Altogether, $\partial_\q \psi(\phi(\q))$ produces an increasing repulsive force as distance to the object decreases, and $\| \qd \| ^2$ makes $\h_2(\q, \qd)$ homogeneous of degree 2 in $\qd$. For this experiment, $\lambda = 0.7$, $k = 0.5$ for two scenarios: 1) $\alpha = 1.5$, and 2) $\alpha = 0.75$. The behavior of this geometry can be seen in Figure \ref{fig:phi2_case1}a. Noticeably, the paths generated are completely overlapping which confirms path consistency.

% Another example of a generator that can produce obstacle avoiding paths is one derived from an energy CHOMP-like Lagrangian \cite{ratliff2009chomp}, $\Lag_e = \frac{1}{2} \psi(\phi(\q)) \|\qd\|^2$ where $\psi(\phi(\q))$ is the same as before. Passing this Lagrangian through the Euler-Lagrange equation produces a corresponding energy tensor and force, $\M_e$ and $\f_e$. These terms can be used to construct an obstacle avoiding geometry as
% \begin{align}
%     \h_2(\q,\qd) = -\M_e^{-1} \f_e.
% \end{align}
% For this experiment, the two scenarios are with $\alpha = 0.75$ and $\alpha = 0.375$. The behavior of this geometry can be seen in Fig. \ref{fig:phi2_case1}b. Again, path consistency among the obstacle avoiding paths is observed.

% A final obstacle-avoiding geometry is constructed by leveraging a Finsler energy. Given a Finsler energy, $\Lag_e = \frac{1}{2 \phi(\q)^2}  (\J(\q) \qd)^2$, a geometry can be constructed as
% \begin{align}
%     \h_2(\q,\qd) = \lambda \Lag_e \: \partial_\q \psi(\phi(\q))
% \end{align}
% where $\phi(q)$ is a differentiable map. This geometry was simulated with $\lambda = 0.7$ for $\alpha = 1.5$ and $\alpha = 0.75$. The paths generated can be seen in Figure \ref{fig:phi2_case1}c. Again, the paths are consistent and this geometry produces an obstacle avoiding behavior. Overall, these three examples illustrate not only path consistency but also the flexibility by which geometries can be designed.

% \begin{figure*}[t]
%   \vspace{2mm}
%   \centering
%   \includegraphics[width=1.\linewidth]{optimization_fabrics/figures/obstacle_geometry.jpg}
%   \vspace{-4mm}
%   \caption{Paths generated from particle motion initiated at different speeds and three different generators. Faded paths indicate higher $\alpha$ and opaque paths indicate lower $\alpha$. Experiment is described in Section \ref{sec:PathConsistencyExperiment}.}
%   \label{fig:phi2_case1}
%   \vspace{-4mm}
% \end{figure*}

% \subsection{Energization commutes with pullback} \label{sec:EnergizationCommutesExperiment}
% Simulations are conducted to empirically demonstrate the theoretical finding that energization cummutes with pullback for full rank systems. Again, the significance of this finding is that leaf generators can be energized in their leaf coordinates and pulled back or pulled back and energized in root coordinates with an equivalent pulled back energy.

% A generator is designed in polar coordinates $\x = [r, \theta ]^T$ for $\ddot{\x} + \h_2(\x, \xd) = 0$ as
% \begin{align}
% \h_2(\x, \xd) = \| \xd \| ^2 \partial_\x \psi(\x)
% \end{align}
% where $\psi(\x) = -\frac{1}{2} \| \x \| ^2$. Effectively, this generator tries to maximize the value of $\| \x \| ^2$ so the trajectories will move such that $r \to \infty$ while $\theta \to \pm \frac{\pi}{2}$. This geometry is separately energized in both the leaf and the root with $\Lag_e = \frac{1}{2} \xd^T \xd$ and produces the exact same behavior in Figure \ref{fig:energization_commutes_2D}. This result empirically confirms that energization commutes with pullback for full rank systems.

% \begin{figure}
%   \vspace{2mm}
%   \centering
%   \includegraphics[width=0.8\linewidth]{optimization_fabrics/figures/energization_commutes_2D.jpg}
%   \vspace{-4mm}
%   \caption{Paths created by a generator and energy built in polar coordinates and pulled back into root coordinates. This result is exactly the same for pulling back the generator first and then energizing in the root. Experiment is described in Section \ref{sec:EnergizationCommutesExperiment}. }
%   \label{fig:energization_commutes_2D}
%   \vspace{-4mm}
% \end{figure}


% \section{Layer-wise construction of geometric fabrics} \label{sec:ComposabilityAndOptimizationExperiment}

% As previously discussed, geometries define underlying behavior and one can conceivably arrive at increasingly richer behavior by composing multiple, individual geometries together as in Proposition \ref{prop:weighted_geometries}. Compositionality, and in particular, \textit{sequential} compositionality, of geometries is a powerful paradigm for building system behavior. For instance, desirable system behavior may include respecting coordinate boundaries, obstacle avoidance, motion bias towards a target location, and ultimately, reaching that target location. Most of these behaviors can be captured as geometries. When energized, the geometries in combination with an attraction potential and damping will achieve the desired system behavior. As subsequently demonstrated, system behavior will be incrementally advanced through the sequential addition of geometrically defined behavior. Numerical results will reveal overall behavior of the underlying geometry and the departure from these natural paths with optimization. Moreover, results will demonstrate increasingly complex system behavior through the addition of geometries and provide empirical evidence that optimization can occur over arbitrary geometries.

% \subsection{Optimization Potential, Speed Control, and Damping Settings} 
% Specific optimization and numerical integration settings that persist throughout the remaining experiments in this section include the following. A set of 14 particles were given initial conditions of $\q_0 = [2, 3]^T$ and $\|\qd_0\| = 1.5$ pointing radially outward and rotationally distributed from $0$ to $2\pi$. Forward integration of system behavior is conducted with the Runge-Kutta fourth-order routine with a maximum step size of 0.01 s for 16 s of simulation time. The optimization potential is an acceleration-based design as discussed in Section \ref{subsec:acceleration_potential} and is designed for the task space
% \begin{align}
% \label{eq:attractor_task_map}
% \x = \phi(\q) = \q - \q_d,
% \end{align}
% where $\q_d$ is the desired position, in this case, $\q_d = [-2.5, -3.75]^T$. The acceleration-based potential gradient, $\partial_\q \psi(\phi(\q)) = M_\psi(\phi(\q)) \partial_\q \psi_1(\phi(\q))$, is designed with
% \begin{align}
% \label{eq:attractor_potential}
% \psi_1(\phi(\q)) = k \left( \|\phi(\q)\| + \frac{1}{\alpha_\psi}\log\big(1 + e^{-2\alpha_\psi \|\phi(\q)\|}\big) \right)
% \end{align}
% and
% \begin{align}
% \label{eq:potential_priority}
% M_\psi(\phi(\q)) = (\widebar{m} - \underline{m}) e^{-(\alpha_m \|\phi(\q)\|) ^ 2} I + \underline{m} I.
% \end{align}
% Furthermore, $k \in \mathbb{R}^+$ is a parameter that controls the overall gradient strength, $\alpha_\psi \in \mathbb{R}^+$ is a parameter that controls the transition rate of $\partial_\q \psi_1(\phi(\q))$ from being nearly a constant to 0. $\widebar{m}$, $\underline{m} \in \mathbb{R}^+$ are the upper and lower isotropic masses, respectively. $\alpha_m \in \mathbb{R}^+$ controls the width of the radial basis function. For the following experiments, $k = 5$, $\alpha_\psi = 10$, $\widebar{m} = 2$, $\underline{m}=0.3$, and $\alpha_m = 0.75$. Importantly, the energy $\Lag_{e,\psi} = \q^T \M_\psi(\phi(\q)) \q $ is added to the system energy, $\Lag_e$. Altogether, this design allows for $\partial_\q \psi(\x)$ to be small far away from the object while smoothly escalating with heightening priority as position towards the target location decreases.

% For these experiments, damping is invoked as discussed in Section \ref{subsec:damping}. Here, $B=6.5$, $\underline{B} = 0.01$, and the switching function is designed as
% \begin{align}
% s_\beta (\x) = \frac{1}{2} (\tanh(-\alpha_\beta (\|\x\| - r) ) + 1) 
% \end{align}
% where $\alpha_\beta \in \mathbb{R}^+$ defines the quickness of the switch, and $r \in \mathbb{R}^+$ defines the radius at which the switch is half-way engaged. For these experiments, $\alpha_\beta = 0.5$ and $r = 1.5$.

% Finally, the switching function $\eta$ from Section \ref{sec:speed_control} that allows to increase system energy for execution energy control is designed as 
% \begin{align}
% \eta = \frac{1}{2} (\tanh(-\alpha_\eta (\Lag_{ex} - \Lag_{ex,d}) - \alpha_{shift} ) + 1) 
% \end{align}
% where $\alpha_\eta$ $\alpha_{shift} \in \mathbb{R}^+$ are parameters that control the quickness of the switch and the horizontal location of the switch, respectively. Moreover, $\Lag_{ex,d}$ is the desired execution energy level. In these experiments, controlling the Euclidean speed, $\|\qd\|$, is desired. Therefore, with a desired Euclidean speed, $v_d$, the execution energy is designed as $\Lag_{ex,d} = \frac{1}{v_d} \qd^T \qd$. Finally, $v_d = 2$ in the following experiments, which is higher than the initialized speed, $\|\qd_0\| = 1.5$.

% \subsection{Layer 1: Baseline Geometry} \label{sec:BaselineOptimizationExperiment}
% An advisable starting point for any system built from geometries is to create a baseline geometry with a non-zero energy tensor (priority) everywhere. Effectively, this ensures that the system always has mass even if other geometries are designed such that their priorities (mass) vanish to zero under desirable conditions. 

% The baseline geometry is constructed from $\h_{2,b} = 0$ and prioritized with an energy tensor, $M_b$, from the Finsler energy, $\Lag_{e,b} = \frac{\lambda_b}{2} \q^T \q$, where $\lambda \in \mathbb{R}^+$ is a parameter that defines the amount of baseline inertia. For these experiments, $\lambda_b = 1$. Therefore, the weighted system geometry and system energy is
% \begin{align}
% \M_e \qdd = \M_b \qdd = \M_b \h_{2,b}
% \end{align}
% and
% \begin{align}
% \Lag_{e} =  \Lag_{e,b},
% \end{align}
% respectively. System behavior can be seen in the first row of Figure \ref{fig:geometries_optimization}. As shown, the underlying geometry results in straight-line motion due to the nature of the Euclidean geometry. During optimization, the motion of particles are redirected from their natural paths resulting in a symmetric plume that terminates at the desired location. Along these paths, particle motion quickly achieves and maintains the desired speed level before the escalation in damping removes energy from the system near the desired location, resulting in convergence to the desired target.


% %%% Figure fig:geometries_optimization was originally here. Moved to accommodate text flow.


% \subsection{Layer 2: Limit Avoidance} \label{sec:LimitOptimizationExperiment}
% A useful task space is often one-dimensional and captures the distance between a current position and some boundary. This task space is generally denoted as $x \in \mathbb{R}$ and subsequently used to describe different one-dimensional distance task spaces. For instance, the distance to an upper and lower coordinate limit can be described as
% \begin{equation}
% \label{eq:upper_limit_map}
% x = \phi(q_j) = \bar{q}_j - q_j
% \end{equation}
% and 
% \begin{equation}
% \label{eq:lower_limit_map}
% x = \phi(q_j) = q_j - \underline{q}_j,
% \end{equation}
% respectively, where $\bar{q}_j$ and $\underline{q}_j$ are the upper and lower limits of the $j^{th}$ coordinate of $\q$. Overall, $2n$ task maps, $x$, are needed for $n$-dimensional coordinates, $\q$. Repulsive geometries can be constructed in this one-dimensional space as
% \begin{align}
% \label{eq:limit_geometry}
% h_{2,i}(x, \dot{x}) = \lambda \dot{x}^2 \partial_{x} \psi(x)
% \end{align}
% where the potential $\psi(x)$ is designed such that $\psi(x) \to \infty$ as $x \to 0$ and $\psi(x) \to 0$ as $x \to \infty$. This potential function is specifically designed here as,
% \begin{align}
% \psi(x) = \frac{\alpha_1}{x^2} + \alpha_2 \log \left(e^{-\alpha_3(x - \alpha_4)} + 1 \right)
% \end{align}

% \begin{figure}
%   \centering
%   \includegraphics[width=.95\columnwidth]{optimization_fabrics/figures/geometries_optimization.jpg}
%   \vspace{-4mm}
%   \caption{\small The left column (a) shows the nominal behavior of the underlying geometric fabric and the right column (b) shows the behavior optimization over it (see Sections \ref{sec:BaselineOptimizationExperiment} - \ref{sec:AttractorOptimizationExperiment} for details on each row). As the fabric complexity grows row-by-row the underlying nominal behavior becomes more sophisticated (left), but optimization (right) remains successful and consistent.}
%   \label{fig:geometries_optimization}
% \end{figure}

% Moreover, $\alpha_1$, $\alpha_2$, $\alpha_3$, $\alpha_4 \in \mathbb{R}^+$ where, $\alpha_1$ and $\alpha_2$ are gains that control the significance and mutual balance of the first and second terms. $\alpha_3$ controls the sharpness of the smooth rectified linear unit (SmoothReLU) while $\alpha_4$ offsets the SmoothReLU. For the following experiments, $\alpha_1 = 0.4$, $\alpha_2 = 0.2$, $\alpha_3 = 20$, and $\alpha_4 = 5$. This potential function offers two key features: 1) a nearly constant gradient force to influence motion farther away from coordinate limits, and 2) an unlimited gradient force as distance to a coordinate limit shrinks, preventing motion from crossing the limit.  

% To establish appropriate priorities for these geometries, individual energy tensors, $M_i$, are created from energies, $\Lag_{e_i}$, where $i=1,...,2n$. $\Lag_{e_i}$ is designed as
% \begin{align}
% \Lag_{e_i} = \frac{1}{2} s(\hat{\dot{x}}) \: G(x) \dot{x}^2
% \end{align}
% where the metric is designed as $G(x) = \frac{\lambda}{x}$ and a switching function $s(\hat{\dot{x}})$ designed as
% \begin{equation}
% s(\hat{\dot{x}}) = 
%     \begin{cases} 
%       0 & \hat{\dot{\phi}}(q_j) \geq 0 \\
%       1 & \hat{\dot{\phi}}(q_j) < 0 \\
%   \end{cases}
% \end{equation}
% Effectively, this removes the effect of the coordinate limit geometry once motion is orthogonal or away from the limit. Finally, to use this geometry within the existing two-dimensional system, all coordinate-limiting geometries must be pulled back to root coordinates, $\q$. The weighted geometries at the root take the form,
% \begin{align}
% \J_i^T M_i \J_i \qdd = -\J_i^T M_i \dot{\J_i} \qd - \J_i^T M_i h_{2,i}.
% \end{align}

% To illustrate the effect of adding this geometry to the system, limits are placed at $\pm 4$ for both $q_1$ and $q_2$, a two-dimensional Euclidean space. Furthermore, $\lambda = 0.25$. Now the total system weighted geometries and system energy is described by
% \begin{align}
% M_e \qdd 
% &= \left( \M_b + \sum_i \J_i^T M_i \J_i \right) \qdd \\
% &= \M_b \h_{2,b} + \sum_i -\J_i^T M_i \dot{\J_i} \qd - \J_i^T M_i h_{2,i}
% \end{align}
% and
% \begin{align}
% \Lag_{e} =  \Lag_{e,b} + \sum_i \Lag_{e,i}
% \end{align}

% The time evolution of the system geometry can be see in the second row of Figure \ref{fig:geometries_optimization}a. If particles are far away from their limits, then straight-line motion is observed due to the underlying Euclidean geometry. As particles approach limit boundaries, repulsion impedes motion towards the limits, and motion is ultimately redirected to limit corners before any one limit is reached. Once energized, optimization was conducted with this geometry as can be seen in Figure \ref{fig:geometries_optimization}b. Importantly, behavior is not significantly influenced when motion is away from limits or distance to limits are larger. Subtle behavioral changes can be seen by the slight bulging of the particle plume and the approach to the target is slightly more aligned with the vertical direction.

% \subsection{Layer 3: Obstacle Avoidance} \label{sec:ObstacleOptimizationExperiment}
% Another canonical behavior is that of obstacle avoidance. This behavior is akin to limit avoidance except the task map is different to accommodate an object instead of a coordinate limit. For instance, the task map for a circular object can be defined as 
% \begin{equation}
% x = \phi(\q) = \frac{\|\q - \q_o\|}{r} - 1
% \end{equation}
% where $\q_o$ is the origin of the circle and $r$ is its radius. A geometry for obstacle avoidance can be constructed with the exact same form as the limit avoidance geometry,
% \begin{align}
% h_{2,o}(x, \dot{x}) = \lambda \dot{x}^2 \partial_x \psi(x)
% \end{align}
% where $\psi(x)$ is the same potential function from limit avoidance. To define priority for this geometry, the same energy structure, switching function, and metric from limit avoidance is leveraged again as well,
% \begin{align}
% \Lag_{e,o} = \frac{1}{2} s(\hat{\dot{x}}) \: G(x) \dot{x}^2.
% \end{align}
% Now, the total weighted system geometry and energy are

% \begin{align}\nonumber
% M_e \qdd
% &= \left( \M_b + \sum_i \J_i^T M_i \J_i + \J_o^T M_o \J_o \right) \qdd \\\nonumber
% &= \M_b \h_{2,b} + \left( \sum_i -\J_i^T M_i \dot{\J_i} \qd - \J_i^T M_i h_{2,i} \right)\\ &\ \ \ \ \ \ -\J_o^T M_o \dot{\J_o} \qd - \J_o^T M_o h_{2,o}
% \end{align}
% and
% \begin{align}
% \Lag_{e} =  \Lag_{e,b} + \sum_i \Lag_{e,i} + \Lag_{e,o}.
% \end{align}

% This combination of geometries and energies produces the behavior seen in the third row of Figure \ref{fig:geometries_optimization}a. Importantly, trajectories that are far from the object do not experience its effect and those closer to the object (magenta and yellow curves) are redirected. The particle belonging to the red curve was directed straight to the object's center and therefore it increasingly slows as it approaches the boundary of the object. The red particle path does subtly redirect around the object as a product of the faint interactions of the limit avoiding geometries.

% Again, optimization is conducted over this increasingly more complex geometric fabric and results are shown in the third row of Figure \ref{fig:geometries_optimization}b. As seen, paths naturally bend around the obstacle and convergence to the target occurs. Importantly, despite the red and cyan curves approaching orthogonally (or nearly so) to the object, they successfully circumnavigate it and optimization succeeds. It is also possible to incorporate different task spaces and geometries to encourage early object avoidance even if the approach direction is orthogonal to the object.

% \subsection{Layer 4: Randomized Vortices} \label{sec:VortexOptimizationExperiment}
% Randomized vortex geometries are added to the system as an abstraction of invoking significant and desired behavioral changes to a system. Furthermore, the vortices create a rather chaotic fabric for optimization, yet, optimization still succeeds as guaranteed by the theory. A vortex geometry is created in root coordinates as
% \begin{align}
% \h_{2,j}(\q, \dot{\q}) = f_j \| \qd \| ^2 \mathbf{R}_j \hat{\qd}
% \end{align}
% where $\mathbf{R}_j \in \mathbb{R}^{2\times 2}$ is a rotation matrix randomly selected as either
% \begin{align}
% \mathbf{R}_j = \pm
% \begin{bmatrix}
% 0 & -1\\
% 1 & 0
% \end{bmatrix}
% \end{align}
% and $f \in \mathbb{R}^+$ is a force magnitude uniformly drawn from the interval $f \sim \mathcal{U}(2, 10)$. A radial priority for this geometry was created from the energy tensor of the following energy,
% \begin{align}
% L_{e,j} = m s(\q) \qd^T \qd
% \end{align}
% where $m \in \mathbb{R}^+$ is a mass constant and the switching function $s(\q) \in [0,1]$ is defined as
% \begin{equation}
%     s(\q) =
%     \left\{ \begin{array}{ll}
%     \frac{1}{\|\q - \q_{o,j}\|^2} (\|\q - \q_{o,j}\| - r)^2 & \|\q - \q_{o,j}\| < r \\
%     0 &\text{otherwise}
%     \end{array} \right.
% \end{equation}
% where $\q_{o,j}$ is the effect center of a vortex and $r \in \mathbb{R}^+$ is its radius. In these experiments, $r=1$ for all vortices.

% The total system weighted geometries and energy is now
% \begin{align}
% M_e \qdd
% &= \left( \M_b + \sum_i \J_i^T M_i \J_i + \J_o^T M_o \J_o + \sum_j \M_j \h_{2,j} \right) \qdd \\
% &= \M_b \h_{2,b} + \sum_i -\J_i^T M_i \dot{\J_i} \qd - \J_i^T M_i h_{2,i} -\J_o^T M_o \dot{\J_o} \qd - \J_o^T M_o h_{2,o} + \\
% & \sum_j \M_j \h_{2,j}
% \end{align}
% and
% \begin{align}
% \Lag_{e} =  \Lag_{e,b} + \sum_i \Lag_{e,i} + \Lag_{e,o} + \sum_j \Lag_{e,j}.
% \end{align}

% As seen in the fourth row Figure \ref{fig:geometries_optimization}a, the addition of vortex geometries create turbulence to the object motion, redirecting particles in different directions as they enter a vortex zone. Despite this volatility, optimization progresses unhindered with all particles making the target location as shown in Figure \ref{fig:geometries_optimization}b. Moreover, the paths taken during optimization are also significantly different from the previous optimization results, showcasing the innate ability of geometries to influence system behavior.

% \subsection{Layer 5: Attractor} \label{sec:AttractorOptimizationExperiment}
% Finally, geometries can also be constructed to facilitate optimization. The previous addition of vortex geometries produced exploratory behavior beyond more straightforward motion to the goal location. However, straight motion to the goal could be desired system behavior. This trait can easily be obtained with the addition of another geometry. Using the same task map of the optimizing potential (Equation \ref{eq:attractor_task_map}) and the potential from Equation \ref{eq:attractor_potential}, an attracting geometry can be constructed as 
% \begin{align}
% \label{eq:att_geometry}
% \h_{2,a} = \lambda_a \| \qd \| ^2 \partial_\q \psi(\phi(\q))
% \end{align}
% where $\lambda_a \in \mathbb{R}^+$ is a control gain. This geometry is prioritized with the energy tensor from the energy,
% \begin{align}
% L_{e,a} = \xd^T \mathbf{G}_a \xd
% \end{align}
% where the metric $\mathbf{G}_a$ is designed as
% \begin{align}
% \mathbf{G}_a = s(\x) (\widebar{m} - \underline{m}) I + \underline{m} I
% \end{align}
% where $\widebar{m}$ and $\underline{m}$ are the upper and lower isotropic mass values and the switching function is designed as
% \begin{align}
% s(\x) = \frac{1}{2} (\tanh(-\alpha_s(\|\x\| - r)) + 1)
% \end{align}
% where $\alpha_s \in \mathbb{R}^+$ controls the rate of the switch and $r$ is the effect radius. Overall, this metric allows the priority to transition from a small to a large isotropic priority as the position nears the target. For these experiments, $\widebar{m} = 1$, $\underline{m} = 0$, $\alpha_s = 25$, $r = 5$, $\lambda_a = 7$. The parameter values for the attracting potential from Equation \ref{eq:attractor_potential} are $k=1$ and $\alpha_\psi=1$. Effectively, this geometry does not engage until the Euclidean distance between the current position and the target is within 5 units.

% Altogether, the system now possesses the total weighted geometry,
% \begin{align}
% M_e \qdd
% &= \left( \M_b + \sum_i \J_i^T M_i \J_i + \J_o^T M_o \J_o + \sum_j \M_j \h_{2,j} + \M_a \right) \qdd \\
% &= \M_b \h_{2,b} + \sum_i -\J_i^T M_i \dot{\J_i} \qd - \J_i^T M_i h_{2,i} -\J_o^T M_o \dot{\J_o} \qd - \J_o^T M_o h_{2,o} + \\
% & \sum_j \M_j \h_{2,j} + \M_a \h_{2,a}
% \end{align}
% and system energy,
% \begin{align}
% \Lag_e = \Lag_{e,b} + \sum_i \Lag_{e_i} + \Lag_{e,o} + \sum_j \Lag_{e,j} +  \Lag_{e,a}.
% \end{align}
% where the individual energies can be pulled back into root coordinates by direct substitution of the task maps and their time derivatives. The total energy Lagrangian can then be passed through the Euler-Lagrange equation to obtain system mass, $\M_e$, and force, $\f_e$. The system geometry behavior can be seen in the last row of Figure \ref{fig:geometries_optimization}a. As seen, the underlying geometry biases motion straight towards the target when within the radial threshold. The significant effect of this geometry can also be seen during optimization (last row Figure \ref{fig:geometries_optimization}b) where motion once dominated by the underlying randomized vortices are now compelled straight towards the object when particle positions are within the radial threshold.

\section{Controlled Particle Experiments} \label{sec:ControlledParticleExperiments}
These experiments validate the theoretical findings and generate insight into the behavioral differences between geometric fabrics and Lagrangian fabrics, and usage of speed control. A set of 14 particles at rest to the right of a circular obstacle are attracted to a point to the left (small square). Behavior is integrated for 15 seconds using a fourth order Runge-Kutta method.

\textbf{Lagrangian Fabrics v.s. Geometric Fabrics:} Denoting Lagrangian fabric terms as $(\Lag_e, \pi_l)_\mathcal{X}$ we design Lagrangian fabric acceleration policies as $\pi_l = -\partial_\x\psi$ using acceleration-based potentials $\psi$. The corresponding geometric fabric terms are $(\Lag_e, \pi_g)$ where $\pi_g = \|\xd\|^2\pi_l$, converting the position-only acceleration policies of the Lagrangian fabric into HD2 geometries for a {\em geometric} fabric simply by multiply by $\|\xd\|^2$. Lagrangian terms are actually all {\em forcing terms} per the categorization in Section~\ref{sec:GeometricFabrics}, whereas these geometric fabric terms add to the fabric, itself, and are, therefore, inherently unbiased. 

Below we describe each fabric term, focusing on describing the geometric fabric terms; Lagrangian fabric terms are derived simply by dropping the velocity scaling factor $\|\xd\|^2$ using the relation $\pi_g = \|\xd\|^2\pi_l$.

% \nathan{Is the information in the Point Attraction and Circular Object Repulsion consistent with the above. Perhaps remove or merge up there? I think this entire section can effectively just be the content in the paragraph above and the experiments section (C).}

% \subsection{End-effector Attraction}
% \label{subsec:point_attraction}
\textbf{End-effector Attraction:} The behavior for pulling the end-effector towards a target location is constructed as follows. The task map is $\x = \phi(\q) = \q - \q_d$, where $\q$, $\q_d \in \mathbb{R}^2$ are the current and desired particle position in Euclidean space. The metric is designed as
\begin{align}
\label{eq:potential_priority}
\G_\psi(\x) = (\widebar{m} - \underline{m}) e^{-(\alpha_m \|\x\|) ^ 2} I + \underline{m} I.
\end{align}
where $\widebar{m}$, $\underline{m}$ are the upper and lower isotropic masses, respectively, and $\alpha_m$ is a constant scalar. The acceleration-based potential gradient, $\partial_\q \psi(\x) = M_\psi(\x) \partial_\q \psi_1(\x)$, is designed with
\begin{align}
\label{eq:attractor_potential}
\psi_1(\x) = k \left( \|\x\| + \frac{1}{\alpha_\psi}\log(1 + e^{-2\alpha_\psi \|\x\|} \right)
\end{align}
where $k$ and and $\alpha_\psi$ are constant scalars. Since our task is to ultimately reach our target location, this behavior is a forcing geometric fabric term (for our geometric fabrics policy) with $\pi = -\partial_\q \psi_1(\x)$.

% For Lagrangian Fabrics, the policy is created from the Lagrangian, $\Lag = \xd^T \G_\psi(\x) \xd - 
% \psi(\x)$. For geometric fabrics, the policy is constructed as $\xdd = -\partial_\x \psi_1(\x)$ and weighted by $\M_\psi(\x)$ from the Finsler energy, $\Lag = \xd^T \G_\psi(\x) \xd$.

% \subsection{Circular Object Repulsion}
% \label{subsec:circular_object_repulsion}
\textbf{Circular Object Repulsion:} Collision avoidance with respect to a circular object is constructed as follows. The task map is $x = \phi(\q) = \frac{\|\q - \q_o\|}{r} - 1$, where $\q_o$ is the origin of the circle and $r$ is its radius. Two different metrics are designed to prioritize this behavior. The first is just a function of position, $G_b (x) = \frac{k_b}{x^2}$, while the second is a function of both position and velocity, $G_b (x, \dot{x}) = s(\dot{x}) \frac{k_b}{x^2}$. Moreover, $k_b$ is a barrier gain and $s(\dot{x})$ is a velocity-based switching function. Specifically, $s(\dot{x}) = 1$ if $\dot{x} < 0$ and $s(\dot{x}) = 0$, otherwise. 
% For these experiments, $k_b = 20$.
The acceleration-based potential gradient, $\partial_\q \psi_b(x) = M_b (x) \partial_\q \psi_{1,b}(x)$, is designed with $\psi_{1,b}(x) = \frac{\alpha_b}{2 x^8}$, where $\alpha_b$ is the barrier gain.
% and $\alpha_b = 1$ for these experiments. 

% For Lagrangian fabrics, the policy is created from either $\Lag = G_b(x) \dot{x}^2 - 
% \psi_b(x)$ or  $\Lag = G_b(x, \dot{x}) \dot{x}^2 - 
% \psi_b(x)$. For geometric fabrics, the policy is $
% \ddot{x} = - s(\dot{x}) \dot{x}^2 \partial_x \psi_{1,b}(x)$. This policy is weighted by $\M_b(x)$ or $\M_b(x, \dot{x})$.

% \subsection{Experiments}
\textbf{Experiment Results:} Speed control is used with the execution energy designed as $\Lag_{ex} = \frac{1}{v_d} \qd^T \qd$, where $v_d$ is the desired Euclidean speed. For both geometric and Lagrangian fabrics, behavior is simulated for $v_d=2,4$, for cases using $G_b(x)$ and $G_b(x, \dot{x})$ (see Fig. \ref{fig:gf_vs_lds_particles}).

\begin{figure}[!t]
  \centering
  \includegraphics[width=.8\linewidth]{geometric_fabrics/figures/lds_vs_gf.jpg}
  \vspace{-4mm}
  \caption{Particle behavior for Lagrangian (left column) and geometric (right column) fabrics of desired speed $v_d=2,4$, in cases using metric design of $G_b(x)$ and $G_b(x, \dot{x})$.}
%   \vspace{-4mm}
  \label{fig:gf_vs_lds_particles}
\end{figure}

All particles successfully circumnavigate the object and reach the the target position. However, the Lagrangian fabrics produce more inconsistent behavior across the speed levels. This is pronounced when using $G_b(x, \dot{x})$ since the velocity gate does not modulate the entire obstacle avoidance policy for Lagrangian fabrics. Instead, the mass of the obstacle avoidance policy vanishes, while components of its force remain. The effect of these forces are amplified when traveling at a higher velocity, producing the ``launching'' artifacts. In contrast, geometric fabrics produce more consistent paths across speed levels without any launching artifacts. Finally, the velocity gate facilitates straight-line motion to the desired location once the obstacle is bypassed. Without this gate the system possesses large mass, impeding motion to the desired location.

Using the same geometric fabric (with obstacle velocity gate) and optimization potential from the previous section, the system is evaluated using: 1) speed control with $v_d=2.5$, and 2) basic damping with $\beta = 4$. The resulting time-speed traces are shown in Fig. \ref{fig:speed_vs_basic}. While both strategies still optimize, basic damping leads to a rather chaotic speed profile over time. In contrast, speed control achieves the desired speed in approximately 1 second and maintains it before damping to the final convergence point.

\begin{figure}[!t]
  \centering
  \includegraphics[width=1.\linewidth]{geometric_fabrics/figures/speed_vs_basic.jpg}
  \vspace{-6mm}
  \caption{Speed profiles over time when optimizing over a geometric fabric with (a) basic damping and (b) speed control.}
  \vspace{-4mm}
  \label{fig:speed_vs_basic}
\end{figure}

% \fi  % Ends full version section
